NSLF-OL: Online Learning of Neural Surface Light Fields alongside Real-time Incremental 3D Reconstruction

Immersive novel view generation is an important technology in the field of graphics and has recently also received attention for operator-based human-robot interaction. However, the involved training is time-consuming, and thus the current test scope is majorly on object capturing. This limits the usage of related models in the robotics community for 3D reconstruction since robots (1) usually only capture a very small range of view directions to surfaces that cause arbitrary predictions on unseen, novel direction, (2) requires real-time algorithms, and (3) work with growing scenes, e.g., in robotic exploration. The paper proposes a novel Neural Surface Light Fields model that copes with the small range of view directions while producing a good result in unseen directions. Exploiting recent encoding techniques, the training of our model is highly efficient. In addition, we design Multiple Asynchronous Neural Agents (MANA), a universal framework to learn each small region in parallel for large-scale growing scenes. Our model learns online the Neural Surface Light Fields (NSLF) aside from real-time 3D reconstruction with a sequential data stream as the shared input. In addition to online training, our model also provides real-time rendering after completing the data stream for visualization. We implement experiments using well-known RGBD indoor datasets, showing the high flexibility to embed our model into real-time 3D reconstruction and demonstrating high-fidelity view synthesis for these scenes. The code is available on github.

==> tex/replica.tex <==
%\begin{table*} [htbp]
%	\begin{adjustwidth}{0pt}{0pt}  
%		\centering
%		{\small
%			\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc}
%				\hline
%				& \multicolumn{2}{c|}{Office0} & \multicolumn{2}{c|}{Office1}  &
%				\multicolumn{2}{c|}{Office2} &
%				\multicolumn{2}{c|}{Office3} &
%				\multicolumn{2}{c|}{Office4} &
%				\multicolumn{2}{c|}{room0} &
%				\multicolumn{2}{c|}{room1} &
%				\multicolumn{2}{c|}{room2}              \\
%				
%				& {\footnotesize HG}
%				& {\footnotesize \textbf{Ours}} 
%				& {\footnotesize HG}
%				& {\footnotesize \textbf{Ours}} \\% & Multi-AFFM & Multi-HG\\
%				\hline
%				PSNR $\uparrow$ 
%				&38.12& 38.13
%				&37.63& 37.85
%				&28.38& 28.57
%				&26.64& 26.89
%				&35.02& 35.17
%				&30.06& 30.20
%				&33.51& 33.47
%				&34.37& 34.35
%				\\
%				SSIM $\uparrow$  & & \textbf{0.913}\\ 
%				LPIPS$_{alex}$ $\downarrow$ &0.295 & \textbf{0.283}\\
%				LPIPS$_{vgg}$$ \downarrow$ & 0.416 &\textbf{0.406}
%				\\
%				\hline
%			\end{tabular} 
%		}
%		\caption {Comparison on Replica sequences.} 
%		\label{tab:comp_rep}
%	\end{adjustwidth}
%\end{table*}


\begin{table}
	\centering
\setlength{\tabcolsep}{0.01em}
\renewcommand{\arraystretch}{.5}
	\begin{tabular}{c||  c c c c }
		\hline
		 \rotatebox{90}{\textbf{Room0}}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room0/0.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room0/633.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room0/798.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room0/1776.png}
		\\ \hline \hline
		\rotatebox{90}{\textbf{Room1}}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room1/34.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room1/239.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room1/401.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room1/637.png}	
		\\ \hline \hline
%		\rotatebox{90}{\textbf{Room2}}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room2/119.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room2/980.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room2/1151.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/room2/1834.png}	
%		\\ \hline \hline
		\rotatebox{90}{\textbf{office0}}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office0/181.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office0/747.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office0/798.png}
		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office0/1840.png}	
		\\ \hline \hline
%		\rotatebox{90}{\textbf{office1}}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office1/390.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office1/734.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office1/1253.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office1/1637.png}
%		\\ \hline \hline
%		\rotatebox{90}{\textbf{office2}}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office2/215.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office2/665.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office2/598.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office2/946.png}
%		\\ \hline \hline
%		\rotatebox{90}{\textbf{office3}}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office3/84.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office3/484.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office3/1374.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office3/1864.png}
%		\\ \hline \hline
%		\rotatebox{90}{\textbf{office4}}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office4/1.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office4/416.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office4/1041.png}
%		&\includegraphics[width=.24\linewidth]{im/exp/indoor/replica/HG/office4/1361.png}
%		\\\hline \hline
	\end{tabular}

	\captionof{figure}{MACA on the 3 scenes of Replica dataset~\cite{straub2019replica}. For each scene, we select four predicted images on corresponding row. For full video demo of 8 scenes, please find our project page$^1$.}
	\label{fig:exp:replica}
\end{table}


